Self-Supervised Person Detection in 2D Range Data using a Calibrated Camera

Deep learning is the essential building block of state-of-the-art person detectors in 2D range data. However, only a few annotated datasets are available for training and testing these deep networks, potentially limiting their performance when deployed in new environments or with different LiDAR models. We propose a method, which uses bounding boxes from an image-based detector (e.g. Faster R-CNN) on a calibrated camera to automatically generate training labels (called pseudo-labels) for 2D LiDAR-based person detectors. Through experiments on the JackRabbot dataset with two detector models, DROW3 and DR-SPAAM, we show that self-supervised detectors, trained or fine-tuned with pseudo-labels, outperform detectors trained only on a different dataset. Combined with robust training techniques, the self-supervised detectors reach a performance close to the ones trained using manual annotations of the target dataset. Our method is an effective way to improve person detectors during deployment without any additional labeling effort, and we release our source code to support relevant robotic applications.

==> Self-Supervised Person Detection in 2D Range Data using a Calibrated Camera/internal_notes.tex <==
\section{Notes 1}

\textbf{Experiments (Mats)}

Results of all experiments we discussed on Monday, 28.9., are available 
under \textit{/globalwork/steinweg/IGPD/Paper\_Experiments}.
Check out readme in that directory for more information.

\textbf{Update Tuesday, 29.9}
\begin{itemize}
    \item Results in Tab. 1 + 2 are updated.
    \item directory \textit{data} contains csv files for training
    splits of DROW, JRDB and JRDB\_Pseudo for Fig. 5
    (distance histogram of xy detections 0-30m)
\end{itemize}


%%%%%%%%%% Original results from Mats' experiments %%%%%%%%%%%%%
% \begin{table}[h!]
% \centering
% \setlength{\tabcolsep}{2.0pt}
% \begin{tabularx}{\linewidth}{l cc YYccYY }
% \toprule 
% &&& \multicolumn{2}{c}{DROW3} &&& \multicolumn{2}{c}{DR-SPAAM} \\
% \cmidrule{4-5} \cmidrule{8-9}
% Supervision &&& $AP_{0.3}$ & $AP_{0.5}$ & & & $AP_{0.3}$ & $AP_{0.5}$  \\ 
% \midrule
% Pre-trained from \cite{Jia20arXiv} &&& 68.3 & 72.3 &&& 66.1 & 70.8 \\
% Pseudo-labels                      &&& 70.5 & 75.6 &&& 68.9 & 73.6 \\
% 3D Annotation                      &&& 80.1 & 83.6 &&& 80.0 & 83.6 \\
% \bottomrule
% \end{tabularx}
% \caption{OLD: Performance of DROW3 and DR-SPAAM detector trained from scratch using different supervision.}
% \end{table}


\subsection{Detector Performance}
 
\subsubsection{Train from scratch}

Table~\ref{table:result_train} reports the performance of DROW3 and DR-SPAAM detector on the evaluation split, trained using either generated labels or the annotated 3D bounding boxes.
Since by design the generated labels do not overlap, we additionally train both detectors using ground truth, yet removing the overlapping samples.
This is accomplished by projecting 3D bounding boxes to image plane and removing boxes with overlapping projections, evaluated using the same $T_{iou}$ threshold for label generation (c.f.~Sec.~\ref{sssec:bbox_selection}).
For baseline comparison, we take the detector models pre-trained on the DROW dataset (from~\cite{Jia20arXiv}) and evaluate them without fine-tuning.

\todo{The results show that}

\begin{table}[h!]
\centering
\setlength{\tabcolsep}{2.0pt}
\begin{tabularx}{\linewidth}{l YYccYY }
\toprule 
& \multicolumn{2}{c}{DROW3} &&& \multicolumn{2}{c}{DR-SPAAM} \\
\cmidrule{2-3} \cmidrule{6-7}
 Supervision & $AP_{0.3}$ & $AP_{0.5}$ & & & $AP_{0.3}$ & $AP_{0.5}$  \\ 
\midrule
Pre-trained from \cite{Jia20arXiv} & 68.3 & 72.3 &&& 66.1 & 70.8 \\
Pseudo-labels                      & 70.5 & 75.6 &&& 68.9 & 73.6 \\
Ground Truth (w/o overlapping)     & 78.8 & 82.2 &&& 79.5 & 82.6 \\
Ground Truth (w/ overlapping)      & 80.1 & 83.6 &&& 80.0 & 83.6 \\
\bottomrule
\end{tabularx}
\caption{Performance of DROW3 and DR-SPAAM detector trained from scratch using different supervision.}
\label{table:result_train}
\end{table}


\begin{table}[]
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
                                      & \multicolumn{2}{l|}{DROW (pre-trained)} & \multicolumn{2}{l|}{DR-SPAAM (pre-trained)} & \multicolumn{2}{l|}{DROW (ground truth)} & \multicolumn{2}{l|}{DROW (pseudo labels)} \\ \hline
Sequence                              & AP 0.3             & AP 0.5             & AP 0.3               & AP 0.5               & AP 0.3              & AP 0.5             & AP 0.3              & AP 0.5              \\ \hline
packard-poster-session-2019-03-20\_1  & 0.8193             & 0.8563             & 0.7665               & 0.8206               & 0.9232              & 0.9461             & 0.8481              & 0.9027              \\ \hline
gates-to-clark-2019-02-28\_1          & 0.7989             & 0.8194             & 0.8234               & 0.8441               & 0.8657              & 0.8903             & 0.7959              & 0.8202              \\ \hline
packard-poster-session-2019-03-20\_0  & 0.8003             & 0.8157             & 0.8043               & 0.8244               & 0.9020              & 0.9154             & 0.8240              & 0.8499              \\ \hline
tressider-2019-03-16\_1               & 0.6466             & 0.6638             & 0.5344               & 0.5506               & 0.8981              & 0.9214             & 0.6810              & 0.7095              \\ \hline
clark-center-2019-02-28\_0            & 0.6877             & 0.7161             & 0.7171               & 0.7459               & 0.7935              & 0.8220             & 0.7249              & 0.7554              \\ \hline
svl-meeting-gates-2-2019-04-08\_1     & 0.5832             & 0.6918             & 0.5608               & 0.6911               & 0.6616              & 0.7241             & 0.5469              & 0.6070              \\ \hline
meyer-green-2019-03-16\_0             & 0.6583             & 0.6809             & 0.6844               & 0.7234               & 0.7613              & 0.7823             & 0.6006              & 0.6266              \\ \hline
gates-159-group-meeting-2019-04-03\_0 & 0.6029             & 0.6645             & 0.5584               & 0.6283               & 0.7704              & 0.8314             & 0.6582              & 0.7486              \\ \hline
huang-2-2019-01-25\_0                 & 0.5714             & 0.6186             & 0.6087               & 0.6512               & 0.7135              & 0.7584             & 0.5983              & 0.6557              \\ \hline
gates-ai-lab-2019-02-08\_0            & 0.4037             & 0.4362             & 0.4066               & 0.4451               & 0.4775              & 0.5376             & 0.2965              & 0.3398              \\ \hline
Total                                 & 0.6833             & 0.7225             & 0.6615               & 0.7078               & 0.8019              & 0.8370             & 0.6883              & 0.7321              \\ \hline
\end{tabular}%
}
\end{table}

\subsubsection{Fine-tune}

During deployment, it is often desired to take a pre-trained detector model and fine-tune it to the specific environment or sensor model.
We simulate such situation by taking pre-trained detectors and fine-tune them on the training split.
The results are recorded in Table~\ref{table:result_ft}.
\todo{The numbers show...}

\begin{table}[h!]
\centering
\setlength{\tabcolsep}{2.0pt}
\begin{tabularx}{\linewidth}{l YYccYY }
\toprule
& \multicolumn{2}{c}{DROW3} &&& \multicolumn{2}{c}{DR-SPAAM} \\
\cmidrule{2-3} \cmidrule{6-7}
  & $AP_{0.3}$ & $AP_{0.5}$ & & & $AP_{0.3}$ & $AP_{0.5}$  \\ 
\midrule
Pre-trained from \cite{Jia20arXiv} (w/o fine-tune) & 68.3 & 72.3 &&& 66.1 & 70.8 \\
Pre-trained from \cite{Jia20arXiv} (w/ fine-tune)  & 00.0 & 00.0 &&& 00.0 & 00.0 \\
\bottomrule
\end{tabularx}
\caption{Performance of pre-trained DROW3 and DR-SPAAM detector with or without fine-tuning.}
\label{table:result_ft}
\end{table}

%%%%%%%%%%%% Old texts %%%%%%%%%%%%%%%%%%%%%%%

% We present three different experiments to investigate the potential of a person detector trained exclusively on pseudo labels in different scenarios. 
% First, we focus on the influence of the label configuration on the training process and compare the performance to that of a detector trained using 3D ground truth. 
% Second, we study the problem of training a person detector for deployment on a mobile robot. 
% To this end, we compare the performance of our method to a detector trained on out-of-domain data from a different laser sensor. 
% Finally, we study the influence of dataset size. 
% As no manual labelling is required for our approach and large labeled datasets are costly to obtain, we consider the effects of increased dataset size to be particularly important for the presented evaluation.

% For all experiments we use the DROW detector and evaluate the performance using the metrics proposed in \cite{Beyer18RAL}. 
% We compute the Average Precision (AP) for association radii of $r_{assoc} = [0.3m, 0.5m]$.

% \subsubsection{Pseudo Label Configurations}

% The purpose of this experiment is to investigate how the statistics of the pseudo dataset influence the training process and the final detection performance. 
% To this end, we propose to evaluate the two parameter combinations of the pseudo label generator presented in Section \ref{ssec:pseudo_label_quality}. 
% Furthermore, we evaluate the performance of a DROW detector trained on the JRDB ground truth which serves as an upper bound for the performance of our image-guided method. 
% To ensure comparability of the results, we train all models for the same number of iterations at a fixed foreground ratio. 
% The results of the experiment are displayed in Table \ref{table:results_label_config}.

% %\Dan{Train four networks with different datasets and evaluate them all on JRDB.
% %1. trained using DROW. 
% %2. using high-precision pseudo-labels.
% %3. using high-recall pseudo-labels.
% %4. using JRDB annotations.
% %The results we are looking for is that 2 and 3 beat 1 and are not very far from 4. 
% %Then the message is two-fold.
% %On one hand, the result shows that our pseudo-label is good enough for training a network from scratch (2 and 3 not far from 4).
% %That means one can just deploy the robot in the wild and it can train itself as long as there is a camera with known extrinsic calibration.
% %On the other hand, the result shows that it is beneficial to use our method and train the detector for specific domain, rather than using a detector trained on other domains (2 and 3 beat 1).
% %All networks should be exposed with the same amount of negative and positive samples during training.
% %Another good result would be 2 beats 3 slightly.
% %Since all networks are exposed to the same amount of samples, the high precision in the labels should lead to better performance.
% %The trade-off of course is the longer training time (to get the same amount of samples, high-precision scheme needs more scans, since each scan will have fewer samples), which will be discussed in the next section.}

% %\Dan{I would not discuss in too much detail about how we do the resampling.
% %People who are interested can look up the code.
% %A sentence saying that we train all networks using the same amount of positive and negative samples should suffice.}

% \begin{table}[h!]
% \centering
% \begin{tabular}{ p{4.2cm} c c c }
% \toprule
% Method && AP$_{0.3}$ & AP$_{0.5}$ \\ 
% \midrule
% Config 1 && 0.6340 & 0.7185 \\
% Config 2 && 0.6278 & 0.7161 \\
% \arrayrulecolor{lightgray}\midrule[0.25pt]\arrayrulecolor{black}
% 3D Ground Truth &&  0.6951 & 0.7837 \\
% \bottomrule
% \end{tabular}
% \caption{Detection accuracy on the JRDB validation split for DROW trained on different configurations of pseudo labels as well as the 3D ground truth. All models were trained for a total of 30.000 iterations at a foreground ration of 0.4. For each configuration the best-performing model was selected based on the $AP_{0.5}$.}
% \label{table:results_label_config}
% \end{table}

% %\subsubsection{Time-performance Tradeoff}

% %\Dan{Train two networks, one using high-precision pseudo-labels and the other using high-recall ones.
% %Train both networks for 1. same amount of samples (same with the previous experiments) and 2. same amount of scans, which translates to same amount of time during deployment.
% %The ideal results is that for same samples, high-precision beats high-recall, but for same amounts, high-recall beats high-precision.
% %So in application, if time is a constrain, use high-recall, otherwise use high-precision.}

% \subsubsection{Domain Adaptation}

% The environment in which 2D range data is collected has a substantial impact on the characteristics of the laser range measurements. 
% For example, background measurements, distance distribution of measured persons and presence of other static and dynamic objects give rise to different dataset statistics. 
% We hypothesize that training a detector in a supervised fashion on a certain dataset and deploying it in an environment with different characteristics might significantly impair detection performance. 
% To verify this assumption we evaluate a detector trained on the DROW dataset on JRDB and compare its performance to the detector trained using pseudo labels only. 
% We propose to train a detector on the DROW dataset from scratch as well as to pre-train it on the DROW dataset and fine-tune on JRDB before evaluating the performance.
% To account for the different sensor configurations, we standardize the training procedure such that the same number of points are used for loss computation at a fixed ratio of foreground and background points. 
% Furthermore, we propose to run the same experiments with JRDB measurements down-sampled by a factor of two before any further processing. 
% This way, we account for the different angular resolution of the sensors and provide results for resolutions of the JRDB scans both, higher and lower, than those of the DROW dataset.
% We train a total of four models, one on the DROW dataset, another one on the DROW dataset which is then fine-tuned on JRDB and two models on JRDB, one using full scans and another one using down-sampled scans.
% The results of the experiment are displayed in Table \ref{table:results_domain_adaptation}. 

% \begin{table}[h!]
% \centering
% \begin{tabular}{ p{2.2cm} c c c c }
% \toprule
% Method & DROW & JRDB & AP$_{0.3}$ & AP$_{0.5}$ \\ 
% \midrule
% DROW & \ding{51} & \ding{55} & 0.4704 (0.5007) & 0.5948 (0.6317) \\
% DROW FT & \ding{51} & \ding{51} & 0.0 & 0.0 \\
% \arrayrulecolor{lightgray}\midrule[0.25pt]\arrayrulecolor{black}
% DROW (stride=1) & \ding{55} & \ding{51} & 0.6340 & 0.7185 \\
% DROW (stride=2) & \ding{55} & \ding{51} & 0.6119 & 0.7088 \\
% \bottomrule
% \end{tabular}
% \caption{Detection accuracy on the JRDB validation split for DROW trained on different datasets. The second and third columns indicate the datasets used for training. All models were trained for a total number of 30.000 iterations at a fixed foreground ratio of $0.4$.}
% \label{table:results_domain_adaptation}
% \end{table}

\subsection{Online Learning}

The issue of dataset size for manually labeled point cloud datasets has been stressed repeatedly throughout this paper. 
To illustrate the potential of essentially unlimited access to training data, we leverage the JRDB test set. 
As the labels for this dataset split are not publicly available, we use the 2D bounding boxes and laser range data to generate additional training data for our image-guided approach. 
By using all 27 sequences of the JRDB test set, we increase the size of our training set from X scans to Y scans. 
We compare the performance of a detector trained on the increased pseudo dataset to the one trained on the JRDB ground truth to see if we can approximate the performance obtained using manually labeled annotations by increasing the size of the dataset. 
The results of the experiment are displayed in Table \ref{table:results_dataset_size}. 

%\Dan{This experiment is interesting.
%Assuming the detector is exposed to unlimited number of scans with pseudo-labels (which is the case in deployment), what will its performance be if we keep training it?
%I speculate that there should be a upper cap somewhere.}

\begin{table}[h!]
\centering
\begin{tabular}{ p{2.5cm} c c c c }
\toprule
Method && Scans & AP$_{0.3}$ & AP$_{0.5}$ \\ 
\midrule
Pseudo Standard && 0 & 00.0 & 00.0 \\
Pseudo Large && 0 & 00.0 & 00.0 \\
\arrayrulecolor{lightgray}\midrule[0.25pt]\arrayrulecolor{black}
3D Ground Truth && 0 & 00.0 & 00.0 \\
\bottomrule
\end{tabular}
\caption{Detection accuracy on the JRDB validation split for DROW trained on different dataset sizes. The second column shows the number of scans in the training dataset.}
\label{table:results_dataset_size}
\end{table}


\begin{table}[h!]
\centering
\setlength{\tabcolsep}{2.0pt}
\begin{tabularx}{\linewidth}{l cc YYccYY }
\toprule 
&&& \multicolumn{2}{c}{DROW3} &&& \multicolumn{2}{c}{DR-SPAAM} \\
\cmidrule{4-5} \cmidrule{8-9}
Supervision &&& $AP_{0.3}$ & $AP_{0.5}$ & & & $AP_{0.3}$ & $AP_{0.5}$  \\ 
\midrule
Pre-trained from \cite{Jia20arXiv} &&& 65.5 & 70.8 &&& 62.5 & 68.3 \\
Pseudo labels &&& 67.2 & 75.2 &&& 69.1 & 76.3 \\
Pseudo labels (remove FP) &&& 69.6 & 76.6 &&& 72.8 & 79.0 \\
Pseudo labels (remove FN) &&& 70.0 & 78.3 &&& 70.3 & 77.4 \\
Pseudo labels (remove FP \& FN) &&& 73.0 & 79.9 &&& 72.2 & 79.1 \\
3D Annotation &&& 76.3 & 82.6 &&& 76.5 & 82.1 \\
\bottomrule
\end{tabularx}
\caption{OLD: before using a longer training schedule. Performance of DROW3 and DR-SPAAM detector trained from scratch using different supervision.}
\label{table:result_train}
\end{table}


==> Self-Supervised Person Detection in 2D Range Data using a Calibrated Camera/items.tex <==
Therefore, we include the foreground ratio and valid ratio as metrics computed on the per-point labels obtained from the pseudo labels following the procedure described in Section \ref{ssec:per_point_targets}. 
The metrics are defined as follows:
\begin{eqnarray}
\eta_{FG} &=& \frac{N_{FG}}{N_{FG} + N_{BG}} \\
\eta_{V} &=& \frac{N_{FG} + N_{BG}}{N_{FG} + N_{BG} + N_{DC}}
\end{eqnarray}
with $N_{FG}$, $N_{BG}$ and $N_{DC}$ being the number of points assigned to foreground, background and "Don't Care"-class, respectively. 
The foreground ratio $\eta_{FG}$ is a measure of the class imbalance and thus important to consider for the loss computation during training. 
The valid ratio $\eta_{V}$ captures the relative reduction of laser points due to discarded 2D detections which should be taken into consideration during training as well.

\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{pics/teaser_image.pdf}
  
  \caption{Illustration of our image-guide labelling method. The top image shows 2D person detections and the associated projections of the laser range measurements. The bottom plot shows the scene from bird's-eye view. The blue bounding boxes correspond to the manually labeled 3D annotations. The yellow circle indicates the computed pseudo label, with all laser points inside the circle being considered as belonging to the person. The robot is shown as a red dot with the beams representing the leftmost and rightmost laser beam projected to the inside of the respective 2D bounding box.}
  \label{fig:teaser}
\end{figure}

Various solutions have been proposed for the task of person detection from 2D LiDAR over the years. From methods based on the clustering of hand-engineered features to deep learning-based detectors, the state-of-the-art performance on challenging datasets has been improved consistently. Recently, the DR-SPAAM detector achieved impressive improvements over prior methods by leveraging a temporal aggregation paradigm to incorporate several scans into the detection process. Thus, the problems associated with the low information of single laser scans can be overcome while retaining real-time computation on the mobile robot. \par

A downside, however, is the limited information content of so-called line point clouds. While they allow for fast computation even on computationally-constrained platforms, the comparably low number of measurements makes the detection problem considerably more challenging.

==> Self-Supervised Person Detection in 2D Range Data using a Calibrated Camera/macros.tex <==
% Adapt these
\newcommand{\ourmethod}{\textcolor{red}{MISSING}}
\newcommand{\ourmethodfull}{\textcolor{red}{Missing name for our method}}

% Comment
\newcommand{\Mats}[1]{{\bf\textcolor{red}{Mats: #1}}}
\newcommand{\Dan}[1]{{\bf\textcolor{red}{Dan: #1}}}
\newcommand{\Bastian}[1]{{\bf\textcolor{red}{Bastian: #1}}}
\newcommand{\Alex}[1]{{\bf\textcolor{red}{Alex: #1}}}
\newcommand{\todo}[1]{\textcolor{red}{\small Todo:\,#1}\PackageWarning{TODO:}{#1!}}
\newcommand{\etal}{{\,\textit{et al.}}}
\newcommand{\grayout}[2]{\textcolor{gray}{Todo: #1 #2}}

% Reference
\newcommand{\refsec}[1]{Sec.~\ref{sec:#1}}
\newcommand{\refchap}[1]{Chapter~\ref{chp:#1}}
\newcommand{\refpart}[1]{Part~\ref{part:#1}}
\newcommand{\refeq}[1]{Eqn.~\ref{eq:#1}}
\newcommand{\reffig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\reftab}[1]{Table~\ref{tab:#1}}

% Convenient
\newcommand{\circlenum}[1]{\raisebox{.5pt}{\textcircled{\raisebox{0pt} {\footnotesize{#1}}}}}
\newcommand{\R}[1]{\underline{R{#1}}}
\newcommand{\parag}[1]{\vspace{-11px}\paragraph{#1}\hspace{-9pt}}
\newcommand{\PAR}[1]{\vskip4pt \noindent {\bf #1~}}  % [Never use](http://tex.stackexchange.com/a/132192)
\newcommand{\PARbegin}[1]{\noindent {\bf #1~}}

\newcommand{\fps}{\,FPS\,}
\newcommand{\bx}{\ensuremath{\mathbf{x}}}
\renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\matr}[1]{\mathbf{#1}}
\newcommand{\set}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\ColorMapCircle}{\ding{108}}
\newcommand{\SubItem}[1]{
    {\setlength\itemindent{15pt} \item[-] #1}
}

\newcommand*\widebar[1]{%
   \hbox{%
     \vbox{%
       \hrule height 0.5pt % The actual bar
       \kern0.3ex%         % Distance between bar and symbol
       \hbox{%
         \kern-0.1em%      % Shortening on the left side
         \ensuremath{#1}%
         \kern-0.1em%      % Shortening on the right side
       }%
     }%
   }%
} 


==> Self-Supervised Person Detection in 2D Range Data using a Calibrated Camera/paper.tex <==
\begin{abstract}
Deep learning is the essential building block of state-of-the-art person detectors in 2D range data.
However, only a few annotated datasets are available for training and testing these deep networks, potentially limiting their performance when deployed in new environments or with different LiDAR models.
We propose a method, which uses bounding boxes from an image-based detector (\textit{e.g.} Faster R-CNN) on a calibrated camera to automatically generate training labels (called \textit{pseudo-labels}) for 2D LiDAR-based person detectors.
Through experiments on the JackRabbot dataset with two detector models, DROW3 and DR-SPAAM, we show that self-supervised detectors, trained or fine-tuned with pseudo-labels, outperform detectors trained only on a different dataset.
Combined with robust training techniques, the self-supervised detectors reach a performance close to the ones trained using manual annotations of the target dataset.
Our method is an effective way to improve person detectors during deployment without any additional labeling effort, and we release our source code to support relevant robotic applications.
\end{abstract}

\section{INTRODUCTION}
\label{sec:introduction}

2D LiDARs provide accurate range measurements with a large field of view, often greater than 200 degrees, at an affordable price, and are a popular sensor choice for many robotic tasks, including person detection.
% Compared to cameras, they are less intrusive on privacy and are thus easier to be deployed \Mats{maybe rather less privacy-intrusive which facilitates deployment}.
While early approaches for detecting persons in 2D range data focused on heuristics with hand-crafted features \cite{Leigh15ICRA,Arras07ICRA},
recent studies used convolutional neural networks and further improved the detection results \cite{Beyer18RAL,Jia20arXiv}.

Deep learning has become an integral part of modern detection algorithms, whether from 2D range data \cite{Beyer18RAL,Jia20arXiv} or images \cite{Tan20CVPR,He17ICCV,Redmon16CVPR,Liu16ECCV,Ren15NIPS}. 
The success of these detectors hinges upon the availability of large and high-quality datasets.
Over the past years, significant effort has gone into labeling images with bounding boxes or segmentation masks, whereas relatively little attention has been given to annotating 2D range data (see~Fig.\,\ref{fig:datasets}).
The few available datasets for 2D LiDARs do not possess enough diversity in terms of the surrounding environments and sensor models.
Networks trained solely on these data may not generalize well at deployment, where both the environment and the sensor specification are likely to differ from those encountered during training.

\begin{figure}[ht]
    \centering
 \includegraphics[width=\linewidth]{pics/tikz/teaser.tikz}
    \caption{
    Only few 2D LiDAR datasets with person annotations exist, while a vast amount of image-based annotations are available.
    We utilize the image-based annotations to train 2D LiDAR-based person detectors by generating pseudo-labels from image-based detections.
    $^*$: Numbers are estimated based on person-per-image statistics of the training set.
    %Image (\protect\tikz \protect\draw[red,fill=red] (0,0) circle (.5ex);) and 2D LiDAR (\protect\tikz \protect\draw[blue,fill=blue] (0,0) rectangle (1.0ex, 1.0ex);) dataset with person annotated.
    %Number of annotations for dataset marked with $^*$ are estimated based on the average person per image, since the test set annotation is not available.
    %JRDB is annotated for 3D point cloud, and only a subset of the annotation is visible to the 2D LiDAR and can be used for training (\textit{c.f.}~Sec.\,\ref{sec:evaluation}).
    }
    \label{fig:datasets}
\end{figure}

To overcome the limitation imposed by insufficient training data,
we propose a method to automatically generate labels for training LiDAR-based person detectors using the output of an image-based detector on a calibrated camera.
Given a person bounding box in an image, our method takes the 2D LiDAR points that fall within the box frustum and uses a clustering algorithm to locate the person in the LiDAR coordinate.
The estimated locations of persons in the scene, as well as a set of negative points, are used as pseudo-labels for training a detector.
This allows a robot to train or fine-tine a laser-based detector in a self-supervised fashion.
We empirically demonstrate the validity of the pseudo-labels and show that they can be used for both training and fine-tuning a 2D LiDAR-based person detector.
Additionally, we experiment with robust training techniques to further improve the detector performance. 
Our method is an effective way to boost the performance of a person detector during deployment without any additional labeling effort, and has great potential for many robotic applications. 
In summary, the main contributions of this work are:
\begin{itemize}
    \item We propose a method to automatically generate pseudo-labels for training 2D LiDAR-based person detectors, leveraging the output of an image-based detector and known extrinsic camera calibration.
    \item We demonstrate that the generated pseudo-labels can be used to train or fine-tune a person detector and experiment with robust training techniques to further improve its performance.     
    \item We release our code, implemented in PyTorch with an easy-to-use detector ROS node, for robotic applications.\footnote{\url{https://github.com/VisualComputingInstitute/2D_lidar_person_detection}} 
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{RELATED WORK}
\label{sec:related_work}

% Person detection from 2D range data has a long standing history in the robotics community.
% While early methods are mainly based on heuristics to find specific shapes in range data, the most common paradigm is to segment a scan into connected segments, compute a set of hand-crafted features for each of these, and finally classify them to create detections~\cite{Arras07ICRA,Pantofaru10ROS,Leigh15ICRA}.
% Common methods can be divided into approaches that detect, and then track, individual legs in order to detect persons \cite{Pantofaru10ROS,Leigh15ICRA}, or approaches that directly aim to include both legs in one segment \cite{Arras07ICRA}.
% Optimally, one would learn the representation of persons directly from data to avoid making such hard design choices. 
% The DROW detector \cite{Beyer16RAL} was the first deep learning based walking aid detector working on 2D range data and was later extended to additionally detect persons \cite{Beyer18RAL}.
% Recently, the DR-SPAAM detector improved upon prior methods by leveraging a temporal aggregation paradigm to incorporate previous scans into the detection process, alleviating the problems associated with the low information of single LiDAR scans while retaining real-time computation on a mobile robotic platform.
\subsection{LiDAR-based Person Detection}
Person detection from 2D range data has a long-standing history in the robotics community.
Early approaches~\cite{Fod02ICRA,Scheutz04IROS,Schulz03IJRR} focus on tracking moving blobs in sequential LiDAR scans.
These blobs are detected using manually engineered heuristics in a non-learning fashion.
Later developments~\cite{Leigh15ICRA,Arras07ICRA,Pantofaru10ROS} improved the detection stage by using supervised learning techniques.
In these approaches, a clustering algorithm is first applied over scan points, using clues like proximity~\cite{Leigh15ICRA} or jump distance~\cite{Arras07ICRA}.
A set of hand-crafted features is then extracted for each cluster, and these features are used to train a simple classifier~(\textit{e.g.}~AdaBoost).
In the case of~\cite{Leigh15ICRA,Pantofaru10ROS}, additional heuristics from tracking are employed to post-process the detected clusters.  

Most recent developments~\cite{Beyer16RAL,Beyer18RAL,Jia20arXiv} use deep learning techniques to detect persons directly from data, without manually engineered heuristics or features.
The DROW detector~\cite{Beyer16RAL} is the first deep learning-based walking aid detector working on 2D range data and was later extended to additionally detect persons~\cite{Beyer18RAL}.
The current state-of-the-art method is the DR-SPAAM detector~\cite{Jia20arXiv}, which leverages a temporal aggregation paradigm to incorporate multiple scans into the detection process, alleviating the problems associated with the low information content in a single LiDAR scan while retaining real-time computation on a mobile robotic platform.


% \subsection{Training from Automatically Generated Labels}
\subsection{Automatic Label Generation}
Supervised learning approaches demand intense effort to manually collect and annotate data for the purpose of training and testing.
Automatic label generation has been attempted to reduce the required labeling effort.
For example, Leigh \etal \cite{Leigh15ICRA} generate positive training examples by positioning a 2D LiDAR in an open environment populated with people and negative examples by moving a LiDAR in an environment devoid of people.
This method limits the training examples to a few simple scenarios and cannot be adapted for dynamic data collection at deployment time.
Aguirre \etal \cite{Aguirre2019IJCIS} use Mask R-CNN~\cite{He17ICCV} with a calibrated RGB-D camera to automatically label 2D LiDAR scans for person detection.
However, no evaluation of the labels' accuracy is performed.
Furthermore, only very simple LiDAR-based person detectors are used and both the training and the evaluation are conducted using (potentially incorrect) generated labels, with no evaluation using real annotated data.
The method also relies on depth measurements from an RGB-D camera, imposing an additional sensor requirement. 
% while they are used for both training and evaluation of the detectors.
% Furthermore, they only explore rather simple LiDAR-based person detectors.%, the applicability of the method on real data remains questionable.
% While at its core our approach is similar, we perform a much more thorough evaluation of our label generation method and show that these can be used to train state-of-the-art models. 
% \Alex{add RGB-D reliance and bad measures of final detector.}
Automatic label generation has also been attempted for 3D LiDARs.
Piewak \etal \cite{Piewak18ECCV} and Wang \etal \cite{Wang19RAL} train point-cloud segmentation networks, using segmentation results on matching pixels as supervision.
% Also for 3D LiDARs approaches for automatic label generation exist.
% Piewak \etal \cite{Piewak18ECCV} project 3D LiDAR points onto camera images for which they computed semantic segmentations in order to create 3D semantic annotations for training.
% Wang \etal \cite{Wang19RAL} use to same idea but apply it to instance segmentation and extend it by defining a joint graph over 2D pixels and 3D points to transfer the labels.

In this work, we propose to automatically generate training data for a 2D LiDAR-based person detector using a calibrated RGB camera and image-based person detections.
Compared to~\cite{Leigh15ICRA}, our pseudo-labels are dynamically generated and do not rely on specific conditions of the environment.
Unlike~\cite{Aguirre2019IJCIS}, our method operates on normal RGB cameras and does not require expensive segmentation on images or pixel-precise calibration between sensors.
% Compared to the 3D LiDAR label generation approaches we work with a single scan line which results in less stable pseudo labels, while we need to generate detection annotations in addition to the per point labels.
We conduct extensive experiments to analyze the quality of pseudo-labels and empirically prove their value for training state-of-the-art person detectors.

\subsection{Learning with Noisy Labels}

Training neural networks with imperfect datasets is becoming an increasingly relevant topic.
Proposed methods range from robust loss functions~\cite{Ghosh17AAAI,Zhang18NIPS,Wang2019ICCV,Menon2020ICLR}, or noise modeling~\cite{xiao2015learning,Goldberger17ICLR,Han18NIPSMasking}, to sample selection~\cite{Pawan10NIPS,Jiang18ICML,Han18NIPS}, or re-weighting samples~\cite{Ren18ICML,Shu19NIPS}.
Regularization techniques~\cite{Srivastava14JMLR,Jindal16ICDM,Menon2020ICLR} have also been shown to reduce the effect of label noise.
For a more thorough study on this topic, we refer readers to surveys~\cite{Zhang16AIR,Algan19arXiv,Song20arXiv}.

In our work, we experiment with the~\textit{partially Huberized cross-entropy loss}~\cite{Menon2020ICLR} and the~\textit{mixup} regularization~\cite{Zhang2018ICLR} to deal with the inherent noise of pseudo-labels.
These two methods were picked for their applicability\textemdash they do not rely on specific noise properties, nor do they impose additional constraints (\textit{e.g.} a small set of clean training data).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Generating Pseudo-Labels}
\label{sec:generating_pseudo_labels}

We use a calibrated camera to generate pseudo-labels for training a 2D LiDAR-based person detector.
These pseudo-labels include the location of persons in the LiDAR coordinate frame $\{(p_{x, i}, p_{y,i})\}_i$, and a set of scan points that belong to the background of the scene.
% mask $M \in \mathds{1}^{N}$ indicating scan points that belong to the background of the scene.

We first use an object detector (\textit{e.g.}~Faster~R-CNN~\cite{Ren15NIPS}) to obtain person bounding boxes.
From all bounding boxes, a subset is selected using the following constraints:
% We select a subset of bounding boxes that satisfy the following three constraints:
%From these bounding boxes we select a subset using the following three criteria:
\begin{itemize}
    \item \textit{classification score} greater than a threshold $T_{c}$,
    \item \textit{aspect ratio}, the ratio between width and height, smaller than $T_{AR}$, 
    \item \textit{overlap ratio}, with any other bounding box is smaller than $T_o$. The overlap ratio is defined as the intersection area divided by the area of the box.
\end{itemize}
The goal is to select boxes from which the location of persons can be confidently extracted, rather than locating \textit{all} persons in the scene (\textit{i.e.}~we favor precision over recall in this step).
% These hyper-parameters should be adjusted depending on the used object detector.
% In this paper, we use $T_{c}=0.75$, $T_{AR}=0.45$, and $T_o=0.4$.

Given a selected bounding box, we estimate the center location $(p_{x,i}, p_{y,i})$ of the person in the LiDAR coordinate frame.
Utilizing the known camera calibration, we project the LiDAR points onto the image and extract points that fall within the bottom half of the bounding box (since the LiDAR is mounted at the height of the lower body).
% This is based on the assumption that the LiDAR sensor is mounted at the height of the lower body and could be adjusted for other recording setups.
These points either correspond to a person or to the background (see~Fig.\,\ref{fig:qualitative_results}).
To localize the person, we first run a $k$-means clustering in the range space with $k=2$, which groups points into a close and a far cluster.
We take the average 2D location of points in the close cluster as the initial estimation, and iteratively refine this estimation using a mean shift procedure with a circular kernel of 0.5~$m$ radius.
The mean shift result is used as the estimated person location.
% To localize the person, we first run a $k$-means clustering in the range space with $k=2$, which groups points into a close and a far cluster.
% Taking the average 2D location of points in the close cluster as the seed, we perform a mean-shift using a circular kernel with a 0.5~$m$ radius.
% The result of mean-shift is used as the estimated person location.
% We then use a mean-shift method to estimate the final person center from the close cluster points.
% Here we use a uniform circular kernel with a radius of 0.5~$m$, starting at the average 2D location of points in the close cluster.
This proposed method assumes that the person belongs to the foreground of the scene and is the dominant object in the cropped LiDAR scan, which is typically satisfied by the content of detection bounding boxes.
% In practice, we found this method to robustly localize a person from their surrounding bounding box.

LiDAR points that do not project to any bounding box (including discarded boxes) are taken as the negative training samples.
For increased robustness, we enlarge the width of each bounding box by a factor of 0.1 when generating the negative samples.
% The resulting 2D person centers can then be used to train a LiDAR-based person detector directly, or further be converted to per point ground truth annotations.
% The LiDAR points near the estimated person centers are used as positive samples and all LiDAR points that do not fall into any bounding box are used as negative samples.
% All remaining points, \ie those that are neither close to an estimated person nor marked as a negative sample, are ignored during training since we cannot reliably determine a pseudo label.
% \todo{This bit is repeated further down, however, there it also discusses a 0.4 - 0.8m range of additional ignore points! Also what happens if two persons stand next to each other? They would cause each other to be ignored.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Person Detection with Pseudo-Labels}

\subsection{DROW3 and DR-SPAAM Detector}

We experiment with two state-of-the-art person detectors, DROW3~\cite{Beyer18RAL} and its successor DR-SPAAM~\cite{Jia20arXiv}.
% They are the only existing deep-learning-based person detectors from 2D LiDAR points and have achieved superior results compared to previous feature-based approaches.
The DROW3 detector takes as input a 2D LiDAR scan, expressed as a one-dimensional vector of range measurements.
For each point, it outputs a classification label and, for the positive points, a location offset to the person center.
This is accomplished by pooling a small window of neighboring points, which are processed by a 1D convolutional neural network.
DR-SPAAM improves upon this approach by introducing a spatial attention and auto-regressive model that integrates temporal information to improve detection performance.
Thus, it requires the input to be a sequence of scans.
We refer readers to~\cite{Beyer18RAL,Jia20arXiv} for more details.

We use the generated pseudo-labels to train DROW3 and DR-SPAAM.
For supervising the classification branch, we use points less than 0.4~$m$ away from an estimated person center $(p_{x}, p_{y})$ as the positive samples, and the marked out background points as the negative samples.
For supervising the regression branch, we use points less than 0.8~$m$ away from an estimated person center.
To increase robustness, we discard pseudo-labels with less than five surrounding positive points.
Points that are neither close to a person nor marked as a background are ignored during training.

% To supervise DROW3 and DR-SPAAM, we use the generated pseudo-labels.
% For positive samples, we use all points less than 0.4~$m$ away from an estimated person center $(p_{x}, p_{y})$ and require that there are at least five points for each person.
% Any pseudo-label with less than five surrounding points is discarded and the surrounding points are ignored during training.
% To increase robustness, points at a distance of 0.4~$m$ to 0.8~$m$ from a person center are excluded from training the classifier but are still included for training the regression branch. 
% The negative points marked out when generating pseudo-labels are used as the negative samples.
% All the remaining points, which are neither close to a person's center nor marked as a background, are ignored during training.

\subsection{Robust Training}

In the default setup, the classification branch of DROW3 and DR-SPAAM is supervised with the cross-entropy loss, which is prone to label noise in the training samples~\cite{Ghosh17AAAI,Wang2019ICCV}.
To limit the influence of wrongly generated pseudo-labels, we resort to robust training techniques.
We experiment with the~\textit{partially Huberized cross-entropy loss}~\cite{Menon2020ICLR}, a more robust loss function, and the~\textit{mixup} regularization~\cite{Zhang2018ICLR}.
% A wrongly labeled sample can create arbitrarily large values \Mats{maybe more specific}, making the classifier prone to label noise~\cite{Ghosh17AAAI,Wang2019ICCV}.
% In this work, we experiment with two robust loss functions: \textit{symmetric cross-entropy loss}~\cite{Wang2019ICCV}, and \textit{partially Huberized cross-entropy loss}~\cite{Menon2020ICLR}, as well as the~\textit{mixup} data augmentation~\cite{Zhang2018ICLR}.

% \subsubsection{Symmetric cross-entropy loss}

% Inspired by the symmetry of the KL-divergence, \cite{Wang2019ICCV}~defined a reverse cross-entropy
% \begin{equation}
%     l_{rce} = -\sum_{k=1}^{K} p(k\vert\mathbf{x}) \, log \, q(k\vert\mathbf{x})
% \end{equation}
% for the predicted and real distribution $p(k\vert\mathbf{x})$ and $q(k\vert\mathbf{x})$,
% and proposed the symmetric cross-entropy loss by combining it with the normal cross-entropy loss
% \begin{equation}
%     l_{sce} = \alpha \cdot l_{ce} + \beta \cdot l_{rce},
% \end{equation}
% weighted by $\alpha$, $\beta$.
% When the label is encoded one-hot (i.e. $q(k\vert\mathbf{x}) \in \{0, 1\}$), $log\,0=A$ is defined to avoid numerical instability, where $A$ is a negative constant.

% For the case of binary classification, the symmetric cross-entropy simplifies to
% \begin{equation}
%     l_{sce} = 
%         \begin{cases} 
%             - \alpha \cdot log(p) - \beta \cdot (1-p) A, & \text{if}\ t=1 \\
%             -\alpha \cdot log(1-p) - \beta \cdot p A, & \text{else.}
%         \end{cases}
% \end{equation}
% In our experiment, we use $\alpha=0.1$, $\beta=0.5$, and $A=-6$, the same parameters as in~\cite{Wang2019ICCV}.

\subsubsection{Partially Huberized cross-entropy loss}

The softmax cross-entropy loss is composed of a base loss (cross-entropy) with a sigmoid link.
Menon \etal \cite{Menon2020ICLR} introduce a composite loss-based gradient clipping, linearizing the base loss beyond a threshold while leaving the sigmoid link untouched.
The overall loss function takes the form:
\begin{equation}
    l = 
        \begin{cases}
            - \tau \cdot p + log(\tau) + 1, & \text{if}\ p\leq\frac{1}{\tau} \\
            - log(p), & \text{else,}
        \end{cases}
\end{equation}
which asymptotically saturates for $p\leq\frac{1}{\tau}$, and was proven to be robust against label noise.
The parameter $\tau$ should be set in proportion with the amount of noise in the training samples. 
In our experiments, we use $\tau=5$.

\subsubsection{Mixup regularization}

Given two training samples $(x_i,y_i)$ and $(x_j,y_j)$, Zhang \etal \cite{Zhang2018ICLR} proposed to construct augmented training samples:
\begin{align*}
    \tilde{x}&=\lambda x_i + (1-\lambda)x_j \\
    \tilde{y}&=\lambda y_i + (1-\lambda)y_j,
\end{align*}
with $\lambda\,{\sim}\,$Beta$(\alpha,\alpha)$ and the parameter $\alpha \in (0,\infty)$ controlling the augmentation strength. 
% This data augmentation technique is termed \textit{mixup}.
Unlike the conventional data augmentation which operates on a single sample (e.g. randomly flipping an image), \textit{mixup} generates virtual samples across training data.
It encourages linear behavior in-between training examples, and was shown to improve generalization of a network and increase its robustness against label noise.

To adapt \textit{mixup} for training a detection network, which includes both classification and regression, we use the following multi-task loss
\begin{equation}
    l_{total} = l_{reg} + (1 - w) \cdot l_{cls} + w \cdot l_{mixup},
\end{equation}
where $l_{reg}$ and $l_{cls}$ are the regression and classification loss without \textit{mixup} regularization, $l_{mixup}$ is the classification loss with \textit{mixup}, and $w$ is a weighting factor.
To avoid additional memory overhead, we split the cost into
\begin{align*}
    l_1 &= l_{reg} + (1 - w) \cdot l_{cls}\\
    l_2 &= w \cdot l_{mixup}
\end{align*}
and perform gradient descent over $l_1$ and $l_2$ sequentially at each training iteration.
In our experiment, we use $w=0.7$ and $\alpha=0.2$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure*}
    \newlength{\imw}
    \setlength{\imw}{0.8cm}
    \newlength{\imh}
    \setlength{\imh}{1.8cm}
    
    \centering
    
    \newcommand{\impairall}[1]{%
        \begin{subfigure}{\imw}%
            \includegraphics[width=\imw,height=\imh]{pics/pl_example/#1_im.pdf}%
        \end{subfigure}%
        \begin{subfigure}{\imh}%
            \includegraphics[width=\imh,height=\imh]{pics/pl_example/#1_pt.pdf}%
        \end{subfigure}%
    }%
    \newcommand{\impair}[1]{\impairall{#1}\hfill}
    \newcommand{\impairend}[1]{\impairall{#1}}
    
    
    \rotatebox[origin=c]{90}{Success}\hspace{2mm}
    \impair{success/000001_12}%
    \impair{success/000004_2}%
    \impair{success/000039_1}%
    \impair{success/000126_0}%
    \impair{success/000248_0}%
    \impairend{success/000314_2}%
    \vspace{2mm}%
    
    \rotatebox[origin=c]{90}{Success}\hspace{2mm}
    \impair{success/000007_14}%
    \impair{success/000067_0}%
    \impair{success/000083_3}%
    \impair{success/000457_2}%
    \impair{success/000534_7}%
    \impairend{success/000656_0}%
    \vspace{2mm}%
    
    \rotatebox[origin=c]{90}{Success}\hspace{2mm}
    \impair{success/000384_1}%
    \impair{success/000437_2}%
    \impair{success/000487_2}%
    \impair{success/000593_1}%
    \impair{success/000650_3}%
    \impairend{success/000921_2}%
    \vspace{2mm}%
    
    \rotatebox[origin=c]{90}{Success}\hspace{2mm}
    \impair{success/000739_0}%
    \impair{success/000781_4}%
    \impair{success/000897_1}%
    \impair{success/000947_3}%
    \impair{success/000977_4}%
    \impairend{success/001020_0}%
    \vspace{2mm}%
    
    \rotatebox[origin=c]{90}{Failure}\hspace{2mm}
    \impair{failure/000431_0}%
    \impair{failure/000458_12}%
    \impair{failure/000250_0}%
    \impair{failure/000629_0}%
    \impair{failure/000677_11}%
    \impairend{failure/001373_1}%
    \vspace{2mm}%
    
    \rotatebox[origin=c]{90}{Failure}\hspace{2mm}
    \impair{failure/000968_2}%
    \impair{failure/000813_5}%
    \impair{failure/000759_3}%
    \impair{failure/000964_0}%
    \impair{failure/000164_2}%
    \impairend{failure/000615_5}%

    \newcommand\drawcross{%
        \begin{tikzpicture}%                                              
            \draw[color=new_blue_dark,line width=1.5pt]%
                (-3pt,0) -- (3pt,0)%
                (0,-3pt) -- (0,3pt);%
        \end{tikzpicture}%
    }   
    
    % \caption{To be viewed in pairs of two, best viewed in color. 
    % Left: Person bounding box from a Faster R-CNN detector, overlaid with LiDAR points. 
    % Color encodes measured distance, red being closest and white being farthest (or failed measurement).
    % Right: The pseudo-label (\raisebox{-0.5mm}{\protect\drawcross{}}) and surrounding LiDAR points within a 0.5 $m$ radius.
    % The bottom two rows demonstrate some common failure cases.
    % From left to right: Column 1-2, heavy occlusion; Column 3-4, background distraction; Column 5, sparse LiDAR points at far distance; 
    % % \Mats{we say we require at least 5 laser points for valid detections. Dan: that is part of the training procedure, not part of pseudo-label generation}
    % Column 6, faulty calibration or synchronization between sensors.}
    \caption{Person detections and the top-down view of the matching pseudo-labels (\raisebox{-0.5mm}{\protect\drawcross{}}) with surrounding LiDAR points (within a 0.5 $m$ radius).
    The LiDAR points are overlaid in the detection images, where the color encodes measured distance with red being closest and white being farthest. 
    % The pseudo-label (\raisebox{-0.5mm}{\protect\drawcross{}}) and surrounding LiDAR points within a 0.5 $m$ radius.
    The bottom two rows demonstrate some failure cases: heavy occlusion (columns 1-2); background distraction (column 3-4); sparse LiDAR points at far distance (column 5); and faulty calibration or synchronization between sensors (column6).}
    \label{fig:qualitative_results}
\end{figure*}


\section{EVALUATION}
\label{sec:evaluation}

We first conduct experiments to validate the quality of the pseudo-labels and then demonstrate their effectiveness for training person detectors.
We present two case studies: training detectors using pseudo-labels with pre-collected data as well as fine-tuning detectors using dynamically generated pseudo-labels.

\subsection{The JackRabbot Dataset (JRDB)}

Our experiments are conducted on the JackRabbot dataset~\cite{Martin2019arXiv}.
The dataset was collected using a mobile robot, the \textit{JackRabbot}, in both indoor and outdoor environments.
It includes point clouds from 3D LiDARs, annotated with 3D bounding boxes for persons, and RGB camera images, annotated with 2D bounding boxes.
Although not directly annotated, the JackRabbot dataset contains scans from two SICK 2D~LiDARs.
These LiDARs were mounted at the height of the lower legs, facing the front and the back of the robot, respectively.
The dataset features a full 360\degree~scan with 1091 points, generated by combining scans from the two LiDARs, which was used as the LiDAR input in our experiments.

For the evaluation of our pseudo-labels and trained detectors, we convert the annotated 3D bounding boxes into 2D LiDAR annotations by using their center as the ground truth location of persons in the scene.
%We used the center of the annotated 3D bounding boxes as the ground truth location of persons in the scene.
Since many 3D bounding boxes are occluded in the view of the 2D LiDARs, we only keep annotations that have at least five points within a 0.5~$m$ radius.

The dataset includes person detections from a Faster R-CNN detector~\cite{Ren15NIPS}, which we use as the input to our pseudo-label generation approach. %our image-based detections.
However, using the included RGB images other detectors can be applied, allowing us to potentially further improve the label quality.
For generating pseudo-labels, we use $T_{c}=0.75$, $T_{AR}=0.45$, and $T_o=0.4$.
% We enlarge the detection bounding boxes by 10\,\%, which results in more robust person center estimates.

The JRDB does not provide a train-validation split and the test set annotations are not publicly available.
Hence, we employ a custom train-test split.
We split the 27 sequences of the original train set into 17 sequences for training and 10 sequences for testing.
Our train-test split is balanced with respect to person detection difficulty (assessed using a pre-trained DROW3 detector) and scene properties (indoor \textit{vs.} outdoor).
We refer readers to the released code for further details.

% \begin{table}[h]
% \centering
% \setlength{\tabcolsep}{2.0pt}
% \begin{tabularx}{\columnwidth}{ lYYY }
% \toprule
% Train Sequence (17 total)       & AP$_{\text{0.5}}$ & Scenario    \\ 
% \midrule
% bytes-cafe-2019-02-07\_0                    & 38.5 & Indoor \\
% clark-center-2019-02-28\_1                  & 73.4 & Outdoor \\
% clark-center-intersection-2019-02-28\_0     & 82.3 & Outdoor \\
% cubberly-auditorium-2019-04-22\_0           & 78.5 & Indoor \\
% forbes-cafe-2019-01-22\_0                   & 62.2 & Indoor \\
% gates-basement-elevators-2019-01-17\_1      & 67.7 & Indoor \\
% hewlett-packard-intersection-2019-01-24\_0  & 30.7 & Outdoor \\
% huang-basement-2019-01-25\_0                & 52.3 & Indoor \\
% huang-lane-2019-02-12\_0                    & 77.2 & Outdoor \\
% jordan-hall-2019-04-22\_0                   & 79.7 & Indoor \\
% memorial-court-2019-03-16\_0                & 82.3 & Outdoor \\
% nvidia-aud-2019-04-18\_0                    & 42.8 & Indoor \\
% packard-poster-session-2019-03-20\_2        & 86.1 & Indoor \\
% stlc-111-2019-04-19\_0                      & 63.8 & Indoor \\
% svl-meeting-gates-2-2019-04-08\_0           & 63.0 & Indoor \\
% tressider-2019-03-16\_0                     & 71.0 & Outdoor \\
% tressider-2019-04-26\_2                     & 79.3 & Indoor \\
% \bottomrule
% \end{tabularx}
% \caption{Details of the customized JRDB train split.}
% \label{table:jrdb_train_split}
% \end{table}

% \begin{table}[ht]
% \centering
% \setlength{\tabcolsep}{2.0pt}
% \begin{tabularx}{\columnwidth}{ lYYY }
% \toprule
% Test Sequence (10 total)      & AP$_{\text{0.5}}$ & Scenario    \\ 
% \midrule
% clark-center-2019-02-28\_0                     & 00.0 & Outdoor \\
% gates-159-group-meeting-2019-04-03\_0          & 00.0 & Indoor \\
% gates-ai-lab-2019-02-08\_0                     & 00.0 & Indoor \\
% gates-to-clark-2019-02-28\_1                   & 00.0 & Outdoor \\
% huang-2-2019-01-25\_0                          & 00.0 & Indoor \\
% meyer-green-2019-03-16\_0                      & 00.0 & Outdoor \\
% packard-poster-session-2019-03-20\_0           & 00.0 & Indoor \\
% packard-poster-session-2019-03-20\_1           & 00.0 & Indoor \\
% svl-meeting-gates-2-2019-04-08\_1              & 00.0 & Indoor \\
% tressider-2019-03-16\_1                        & 00.0 & Outdoor \\
% \bottomrule
% \end{tabularx}
% \caption{Details of the customized JRDB test split. \todo{update AP, scenario}}
% \label{table:jrdb_test_split}
% \end{table}


% \textbf{The DROW dataset \cite{Beyer18RAL}} is recorded in an indoor rehabilitation facility using a SICK S300 scanner mounted at 37 cm height.
% Each scan contains 450 range measurements, covering a field of view of 225\degree.
% The dataset is annotated with center location of three classes: wheelchair, people with walking aids, and persons.
% In this experiments, we focus on person detection and ignore annotations of the other two classes.

\subsection{Pseudo-Label Statistics}
\label{ssec:pseudo_label_quality}

To evaluate the quality of our pseudo-labels, we calculate the true positive and the true negative rate (TPR, TNR) of the classification target generated using pseudo-labels by comparing them against the target generated using ground truth annotations.
More than 90 percent of the training samples are labeled correctly (see~Table\,\ref{table:pl_pr_tnr}), indicating the validity of the pseudo-labels.
Qualitative results of pseudo-labels are shown in~Fig.\,\ref{fig:qualitative_results}.
In most cases, locations of persons are successfully estimated in both indoor and outdoor environments, with people at different distances or having different poses.
Common failure cases are based on occluding objects, persons merging with the background, sparse LiDAR measurements at high distances, or a faulty calibration between sensors.
These cases result in noisy labels, which we deal with by using a robust training loss.
% Compared to the negative samples, the positive samples have a slightly lower accuracy.
% This is caused by common failure scenarios such as heavy occlusion, sparse LiDAR points at far distance, or faulty calibration between sensors.
% which is likely due to the common failure scenarios discussed in~Fig.\,\ref{fig:qualitative_results}.

% \begin{table}[b]
% \centering
% \setlength{\tabcolsep}{2.0pt}
% \begin{tabularx}{\columnwidth}{ lYYYY }
% \toprule
% Bounding Boxes      & TPR & TNR & Precision & Recall    \\ 
% \midrule
% Faster R-CNN Detections   & 91.6 & 99.4 & 78.5 & 35.5 \\
% 2D Annotations      & 90.6 & 99.1 & 74.7 & 40.2 \\
% \bottomrule
% \end{tabularx}
% \caption{Pseudo-label evaluation on our training set using different 2D bounding box sources.}
% \label{table:pl_pr_tnr}
% \end{table}

\begin{table}[b]
\centering
\setlength{\tabcolsep}{2.0pt}
\begin{tabularx}{0.8\columnwidth}{ l ccc YY }
\toprule
Bounding Boxes      &&&& TPR & TNR  \\ 
\midrule
Faster R-CNN Detections   &&&& 91.6 & 99.4\\
2D Annotations      &&&& 90.6 & 99.1\\
\bottomrule
\end{tabularx}
\caption{Accuracy of pseudo-labels on the training split.}
\label{table:pl_pr_tnr}
\end{table}

% Since LiDARs scan only the front surface of an object, in most cases there exists a small offset between the pseudo-label location, estimated as the average location of scan points (Sec.\,\ref{sec:generating_pseudo_labels}), and the center of a person.
% To study the localization quality of pseudo-labels, we computed the precision and recall of the estimated person locations.
% An estimated person is regarded as a true positive if there is a ground truth annotation within a 0.5~$m$ association radius.
% % 78.5 percent of all pseudo-labels fell within a 0.5~$m$ radius from an annotation, showing that most pseudo-labels are well-localized for training a detection network.
% Most pseudo-labels are well-localized for training a detection network, as shown by the 78.5 percent precision.
% The remaining 21.5 percent stem from either false pseudo-labels or localization inaccuracy.
% Despite the strict selection criteria enforced on detection boxes, pseudo-labels still cover a significant amount of persons in the scene, as shown by the 35.5 percent recall. 

To ablate the effect of uncertainty in the image-based person detector, we generate pseudo-labels using the annotated 2D bounding boxes.
The TPR and TNR of the pseudo-labels generated using detections are higher than those generated using annotations, showing that our proposed method is robust against uncertainty in bounding boxes.
Due to the sparsity of LiDAR points, it is difficult to generate pseudo-labels for far away persons contained in 2D annotations.
When using a detector, these persons are often missed or detected with low confidence, thus not leading to a (potentially false) pseudo-label.
% Pseudo-labels generated using annotations have higher recall, but lower precision.
% This trade-off comes from far away persons contained in 2D annotations, whose location is hard to accurately determine due to the sparsity of LiDAR points.
% When using a detector, these persons are often missed or detected with low confidence due to their small appearance, thus resulting in no pseudo-label and ultimately a higher precision.

We also analyze the distance distribution of our pseudo-labels.
As Fig.\,\ref{fig:pl_dist} shows, it is similar to that of the annotations.
Pseudo-labels do not introduce any distance bias which may wrongly emphasize samples within a certain range.
Due to the high mounting of cameras in the JackRabbot dataset, the legs of persons close to the robot are outside the camera's field of view.
Thus, no pseudo-label can be generated within 1~$m$ distance.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{pics/distance_histogram.png}
%     \caption{Distance distribution of the generated labels and the annotated 3D bounding boxes.}
%     \label{fig:pl_dist_old}
% \end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{pics/tikz/hist.tikz}%
    \caption{
    Distance distribution of pseudo-labels and annotations.
    Pseudo-labels have a similar distance distribution to that of the annotations and do not introduce a distance bias.
    }%
    \label{fig:pl_dist}%
\end{figure}

\subsection{Training with Pseudo-Labels}
\label{sec:offline_training}

We examine the performance of detectors trained using either pseudo-labels or ground truth annotations.
We train the DROW3 detector for 40 epochs, using a batch size of 8 scans and the DR-SPAAM detector for 20 epochs, using a batch size of 4 scans,
We use the Adam optimizer~\cite{Kingma15ICLR}, and a learning rate of $10^{-3}$.
Starting from 10 epochs for DROW3 and 5 epochs for DR-SPAAM, we exponentially decay the learning rate until it reaches $10^{-6}$ at the end of training.
% For DROW3 we use a burn-in period of 10 epochs, and for DR-SPAAM 5 epochs.
Implementation and hyper-parameters are taken from~\cite{Jia20arXiv} for both detectors, with the only exception being that we enlarge the spatial window size for DR-SPAAM to 17 points (from the original 11 points).
This enlarged window matches the effective opening angles, since the scans in JRDB have a higher angular resolution.
Due to GPU memory constraints, we randomly crop the scans to 1000 points for DR-SPAAM at training time.

We report the average precision (AP$_{\text{0.3}}$ and AP$_{\text{0.5}}$) on the test split (see~Table\,\ref{table:result_train}).
A detection is considered positive if there is a ground truth within 0.3~$m$ or 0.5~$m$, and a ground truth can only be matched with a single detection.
As baselines, we evaluate the released DROW3 and DR-SPAAM model from~\cite{Jia20arXiv}, which is trained on the DROW dataset.
These pre-trained networks have significantly lower AP compared to the ones trained on JRDB, confirming our initial speculation that networks trained on a single dataset may not generalize well to new environments or different LiDAR models.
The pre-trained DR-SPAAM, despite having a higher score on the DROW dataset, performed worse than DROW3, showing the effect of overfitting.
Networks trained using pseudo-labels, benefiting from a smaller domain gap to the test data, outperform the pre-trained networks, proving the validity of our approach.
Starting from a pre-trained model improves the detector performances for pseudo-labels, but gives no clear improvement for 3D annotations.

% In Table\,\ref{table:result_train}, we report average precision (AP) evaluated with a 0.3~$m$ and 0.5~$m$ association radius on our test split.
% The benefit of training with pseudo-labels is evident from the results.
% Networks trained using pseudo-labels have improved performance (6.5 and 7.2 percent higher AP$_{\text{0.5}}$ for DROW3 and DR-SPAAM, respectively), compared to those only pre-trained on a different dataset.
% This higher performance likely comes from the smaller domain gap between pseudo-labels and the testing data given that they were collected using the same sensor setup.
% DR-SPAAM, pre-trained or trained with pseudo-labels, has lower performance compared to DROW3.
% This is likely due to the fact that being a stronger model, DR-SPAAM is more prone to overfitting, whether to a specific dataset or to noise.
% When trained using annotations, DR-SPAAM surpasses the DROW3 performance.

The performance gap between pseudo-labels and annotations could be caused by two factors: label noise and less training samples.
To study the effect of label noise, we additionally train networks with pseudo-labels, while removing falsely labeled points and correcting the regression target using ground truth annotations (see~Table\,\ref{table:result_train_pl}).
% Four experiments were conducted: removing only false positives, only false negatives, and removing both, from the pseudo-labels (see~Table\,\ref{table:result_train_pl}).
Both false positives and false negatives reduce the detector performance, with the later having a strong influence on DROW3.
Correcting the regression target improves AP$_\text{0.3}$ for both networks, especially for the more powerful DR-SPAAM.
Cleaning pseudo-labels increases detector performance significantly, showing that label noise is the more dominant cause to the performance gap between pseudo-labels and annotations.
Detectors trained using clean pseudo-labels trail the ones trained using annotations by around 2 percent AP, due to reduced amounts of training samples.
Fine-tuning with a pre-trained model further narrows this performance gap.

% In addition, the localization inaccuracy in pseudo-labels effect DR-SPAAM significantly.
% By removing false training labels, DROW3 and DR-SPAAM gain an additional 3.5 and 3.3 percent AP$_{\text{0.5}}$, respectively.
% There is still a difference to the networks trained using annotations though, but the gap is significantly smaller compared to that of pre-trained networks.
% If the damage \Mats{damage sounds weird} of labeling noise can be mitigated, training using pseudo-labels can in theory produce detectors with similar performance to those trained using annotations.

% \begin{table}
% \centering
% \setlength{\tabcolsep}{2.0pt}
% \begin{tabularx}{\linewidth}{l cc YYccYY }
% \toprule 
% &&& \multicolumn{2}{c}{DROW3} &&& \multicolumn{2}{c}{DR-SPAAM} \\
% \cmidrule{4-5} \cmidrule{8-9}
% Supervision &&& AP$_{\text{0.3}}$ & AP$_{\text{0.5}}$ & & & AP$_{\text{0.3}}$ & AP$_{\text{0.5}}$  \\ 
% \midrule
% Pre-trained from \cite{Jia20arXiv} &&& 65.5 & 70.8 &&& 62.5 & 68.3 \\
% Pseudo-labels &&& 68.5 & 77.3 &&& 66.9 & 75.5 \\
% \quad + fine-tuning from \cite{Jia20arXiv} &&& 69.0 & 77.8 &&& 69.2 & 76.7 \\
% 3D Annotation &&& 76.2 & \textbf{82.9} &&& 78.5 & \textbf{84.9} \\
% \quad + fine-tuning from \cite{Jia20arXiv} &&& \textbf{76.4} & 82.5 &&& \textbf{78.6} & 83.8 \\
% \midrule
% Pseudo-labels (remove FP) &&& 71.6 & 79.0 &&& 71.1 & 77.8 \\
% Pseudo-labels (remove FN) &&& 68.4 & 77.8 &&& 70.3 & 78.6 \\
% Pseudo-labels (remove FP \& FN) &&& 73.1 & 80.8 &&& 72.2 & 78.8 \\
% \quad + fine-tuning from \cite{Jia20arXiv} &&& \textbf{73.3} & \textbf{80.9} &&& \textbf{73.5} & \textbf{80.9} \\
% \bottomrule
% \end{tabularx}
% \caption{Performance of DROW3 and DR-SPAAM detector trained using different supervision.}
% \label{table:result_train}
% \end{table}

\begin{table}
\centering
\setlength{\tabcolsep}{2.0pt}
\begin{tabularx}{\linewidth}{l cc YYccYY }
\toprule 
&&& \multicolumn{2}{c}{DROW3} &&& \multicolumn{2}{c}{DR-SPAAM} \\
\cmidrule{4-5} \cmidrule{8-9}
Supervision &&& AP$_{\text{0.3}}$ & AP$_{\text{0.5}}$ & & & AP$_{\text{0.3}}$ & AP$_{\text{0.5}}$  \\ 
\midrule
Pre-trained from \cite{Jia20arXiv} &&& 65.5 & 70.8 &&& 62.5 & 68.3 \\
Pseudo-labels &&& 68.5 & 77.3 &&& 66.9 & 75.5 \\
\quad + fine-tuning from \cite{Jia20arXiv} &&& 69.0 & 77.8 &&& 69.2 & 76.7 \\
3D Annotation &&& 76.2 & \textbf{82.9} &&& 78.5 & \textbf{84.9} \\
\quad + fine-tuning from \cite{Jia20arXiv} &&& \textbf{76.4} & 82.5 &&& \textbf{78.6} & 83.8 \\
\bottomrule
\end{tabularx}
\caption{Performance of DROW3 and DR-SPAAM trained using different supervision.}
\label{table:result_train}
\end{table}

\begin{table}
\centering
\setlength{\tabcolsep}{2.0pt}
\begin{tabularx}{\linewidth}{l c YYccYY }
\toprule 
&& \multicolumn{2}{c}{DROW3} && \multicolumn{2}{c}{DR-SPAAM} \\
\cmidrule{3-4} \cmidrule{6-7}
Supervision && AP$_{\text{0.3}}$ & AP$_{\text{0.5}}$ && AP$_{\text{0.3}}$ & AP$_{\text{0.5}}$  \\ 
\midrule
Pseudo-labels && 68.5 & 77.3 && 66.9 & 75.5 \\
$\ldots$ (remove FP) && 71.6 & 79.0 && 71.1 & 77.8 \\
$\ldots$ (remove FN) && 68.4 & 77.8 && 70.3 & 78.6 \\
$\ldots$ (remove FP \& FN) && 73.1 & 80.8 && 72.2 & 78.8 \\
$\ldots$ (remove FP \& FN, correct reg.) && 74.6 & 80.5 && \textbf{76.5} & \textbf{81.5} \\
\quad + fine-tuning from \cite{Jia20arXiv} && \textbf{74.7} & \textbf{81.2} && 76.2 & \textbf{81.5} \\
\bottomrule
\end{tabularx}
\caption{Performance of DROW3 and DR-SPAAM trained with different variants of pseudo-labels.}
\label{table:result_train_pl}
\end{table}

\begin{table}
\centering
\setlength{\tabcolsep}{2.0pt}
\begin{tabularx}{\linewidth}{l cc YYccYY }
\toprule 
&&& \multicolumn{2}{c}{DROW3} &&& \multicolumn{2}{c}{DR-SPAAM} \\
\cmidrule{4-5} \cmidrule{8-9}
Training scheme &&& AP$_{\text{0.3}}$ & AP$_{\text{0.5}}$ & & & AP$_{\text{0.3}}$ & AP$_{\text{0.5}}$  \\ 
\midrule
Cross-entropy loss &&& 68.5 & 77.3 &&& 66.9 & 75.5 \\
\quad + mixup regularization &&& 69.5 & 78.0 &&& 65.8 & 74.0 \\[0.1cm]
% Symmetric cross-entropy loss &&& 62.7 & 72.2 &&& 63.4 & 72.9 \\
% \quad + mixup regularization &&& 61.1 & 69.8 &&& 62.1 & 71.3 \\[0.1cm]
Partially Huberized cross-entropy loss &&& \textbf{71.4} & \textbf{79.0} &&& 69.4 & 76.4 \\
\quad + mixup regularization &&& 71.1 & 78.5 &&& \textbf{70.0} & \textbf{78.3} \\
\bottomrule
\end{tabularx}
\caption{Performance of DROW3/DR-SPAAM trained with pseudo-labels and different robust training methods.}
\label{table:result_robust}
\end{table}

% \noindent \textbf{Robust Training} 
To mitigate the problem caused by labeling noise, we experiment with two robust training methods: the \textit{partially Huberized cross-entropy loss}, and the \textit{mixup} regularization (see~Table\,\ref{table:result_robust}).
Both methods improve the network performance, with the exception of applying \textit{mixup} alone on DR-SPAAM (potentially due to suboptimal hyper-parameters).
Combined with robust training methods, detectors trained using pseudo-labels outperform the pre-trained detectors by a large margin, and reach a performance close to training using annotations, without using any labeled data.
Pseudo-labels provide an effective way to adjust person detectors to new environments or LiDAR models.

% For DROW3, performance improves with both methods, either applied separately or in combination.
% For DR-SPAAM, applying \textit{mixup} alone reduced performance 
% The best performance was using the \textit{partially Huberized cross-entropy loss} alone, reaching 79.0 percent AP$_{0.5}$, 1.7 percent higher than the cross-entropy loss baseline.
% It is 8.2 percent higher than the performance of the pre-trained DROW3 detector, and is only 3.9 percent lower than that of the detector trained using annotations.
% For the DR-SPAAM detector, the best performance is gained using the \textit{partially Huberized cross-entropy loss} together with \textit{mixup} regularization, reaching 78.3 percent AP$_{0.5}$.
% It is 2.8 percent higher than its baseline, but still lower than the DROW3 performance.
% In some combinations, the \textit{mixup} regularization reduces the detector performance, potentially caused by suboptimal hyper-parameters.
% \todo{write about mixed mixup results, say there is potential, however, proper hyperparameter-selection is needed.}


\subsection{Online Fine-Tuning with Pseudo-Labels}

In practice, it is desirable to use a detector that can dynamically fine-tune itself in an online fashion during deployment.
To study the network performance undergoing such fine-tuning, we take a DROW3 detector, pre-trained on DROW dataset~\cite{Jia20arXiv}, and fine-tune it on the JRDB train split for one epoch, with the partially Huberized cross-entropy loss.
We use a learning rate of $5\times10^{-5}$ and a batch size of 8 scans.
In the first set of experiments, we shuffle data only within each sequence (the whole train split is composed of 17 sequences) and pass the in-sequence shuffled data to the network.
This mimics the situation where a mobile robot enters into a new environment, curates a small amount of data, and fine-tunes itself.
% Each sequence on average contains 1000 scans, recorded in a window of two minutes.
In the second set of experiments, we shuffle data within the whole training split, giving more diversity in each batch.
% We fine-tune detectors using both pseudo-labels and the annotations for both sets of experiments.

The detector performance at different stages of fine-tuning is shown in~Fig.\,\ref{fig:online_training}.
When the data is shuffled within the whole training split, the network performance increases significantly, from the pre-trained 70.8 percent AP$_{\text{0.5}}$ to more than 74 percent, using less than one hundred updates.
This fast performance increase implies that, even in applications with insufficient computation for a full training, it is still possible to adapt the detector and improve its performance, by running a small number of updates using pseudo-labels.
However, having curated training samples with enough diversity is a key prerequisite, as fluctuating performance is observed when the data was shuffled only within each sequence.
Although for most of the time the detector benefits from fine-tuning (having better performance than that of a pre-trained detector), there are adversarial samples that cause dramatic performance reductions.
The same fluctuating behavior exists for fine-tuning using annotations, showing that it is an innate problem of network training, rather than caused by pseudo-labels.
Curriculum learning methods~\cite{Bengio09ICML,Jiang18ICML} may help mitigating this problem, and thus relaxing the requirement of data collection. 
They are interesting directions to be explored in future research.


% Main points to discuss:
% \begin{itemize}
%     \item Point out the used loss and issues with the hyperparameters.
%     \item Training on sequence level strongly depends on quality of sequence and is outperformed by full dataset shuffling. It still slightly improves though.
%     \item Even now this can be used to tune a robot on the fly (per sequence). Or it could collect data during the day and train on it during the night (full dataset)
%     \item Full fine-tuning works even better, but training for a short time already works! (Move to table II discussion likely!)
%     \item (maybe) Drow results decrease, but that is in line with the general known problem of forgetting when fine-tuning.
%     \item Discuss the difference between pseudo and 3D box based labels.
% \end{itemize}
% Future work:
% \begin{itemize}
%     \item It depends a lot on the quality of the sequence (shown in plot). Being able to determine this would help.
%     \item Determining some good training curriculum would improve.
%     \item Maybe only train on hard examples that don't match the detections or gather some list of expressive samples to keep in some training/evaluation buffer.
%     \item Lots of potential!
% \end{itemize}

\begin{figure}
    \newcommand\drawdashedline{%
        \begin{tikzpicture}%                                              
            \draw[gray, dashed, line width=0.75pt]%
                (-7.5pt,0) -- (7.5pt,0);%
                % (0,-3pt) -- (0,3pt);%
        \end{tikzpicture}%
    }   
    \centering
    \includegraphics[width=\linewidth]{pics/tikz/online_training.tikz}
    \caption{
    Performance at different steps of fine-tuning a pre-trained DROW3 detector with partially Huberized cross-entropy loss.
    Data is shuffled either on the whole training set or within each sequence, mimicking different amounts of curated data.
    % The pre-trained model has a 70.8 percent AP$_\text{0.5}$ initially (\raisebox{2pt}{\protect \drawdashedline{}}).
    With diverse batches, the detector performance improves significantly even with only a small number of updates.
    Fine-tuning longer using the default training schedule yields 79.2 and 82.3 percent AP$_\text{0.5}$ for pseudo-labels and annotations, respectively.  
    % Fine-tuning longer (as in~Sect.\,\ref{sec:offline_training}) using pseudo-labels and annotations yields 79.2 and 82.3 percent AP$_\text{0.5}$ respectively.  
    }
    
    
    \label{fig:online_training}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{CONCLUSION}

In this paper, we proposed a method to automatically generate pseudo-labels for training 2D LiDAR-based person detectors, using bounding boxes generated from an image-based person detector with a calibrated camera.
We analyzed the quality of pseudo-labels by comparing them against ground truth annotations and proved their validity.
Experiments were conducted to train or fine-tune DROW3 and DR-SPAAM detectors using pseudo-labels, and these self-supervised detectors outperformed the detectors trained on annotations using a different dataset.
Even stronger detectors were obtained by combining pseudo-labels with robust training techniques.

Our method provides an effective way to bridge the domain gap between data encountered during training and during deployment.
With our method, a mobile robot equipped with a 2D LiDAR-based person detector can fine-tune the detector during deployment, improving its performance with no additional labeling effort.
With the released code, we expect our method will be useful for many robotic applications.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Acknowledgements:}

We thank Hamid Rezatofighi, JunYoung Gwak, and Mihir Patel for their help with the JackRabbot dataset.
This project was funded by the EU H2020 project "CROWDBOT" (779942). 
Most experiments were performed on the RWTH Aachen University CLAIX 2018 GPU Cluster (rwth0485).

==> items.tex <==
Therefore, we include the foreground ratio and valid ratio as metrics computed on the per-point labels obtained from the pseudo labels following the procedure described in Section \ref{ssec:per_point_targets}. 
The metrics are defined as follows:
\begin{eqnarray}
\eta_{FG} &=& \frac{N_{FG}}{N_{FG} + N_{BG}} \\
\eta_{V} &=& \frac{N_{FG} + N_{BG}}{N_{FG} + N_{BG} + N_{DC}}
\end{eqnarray}
with $N_{FG}$, $N_{BG}$ and $N_{DC}$ being the number of points assigned to foreground, background and "Don't Care"-class, respectively. 
The foreground ratio $\eta_{FG}$ is a measure of the class imbalance and thus important to consider for the loss computation during training. 
The valid ratio $\eta_{V}$ captures the relative reduction of laser points due to discarded 2D detections which should be taken into consideration during training as well.

\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{pics/teaser_image.pdf}
  
  \caption{Illustration of our image-guide labelling method. The top image shows 2D person detections and the associated projections of the laser range measurements. The bottom plot shows the scene from bird's-eye view. The blue bounding boxes correspond to the manually labeled 3D annotations. The yellow circle indicates the computed pseudo label, with all laser points inside the circle being considered as belonging to the person. The robot is shown as a red dot with the beams representing the leftmost and rightmost laser beam projected to the inside of the respective 2D bounding box.}
  \label{fig:teaser}
\end{figure}

Various solutions have been proposed for the task of person detection from 2D LiDAR over the years. From methods based on the clustering of hand-engineered features to deep learning-based detectors, the state-of-the-art performance on challenging datasets has been improved consistently. Recently, the DR-SPAAM detector achieved impressive improvements over prior methods by leveraging a temporal aggregation paradigm to incorporate several scans into the detection process. Thus, the problems associated with the low information of single laser scans can be overcome while retaining real-time computation on the mobile robot. \par

A downside, however, is the limited information content of so-called line point clouds. While they allow for fast computation even on computationally-constrained platforms, the comparably low number of measurements makes the detection problem considerably more challenging.
